Results from the DM-Ice17 Dark Matter Experiment at the South Pole

DM-Ice is a phased experimental program using low-background NaI(Tl) crystals with the aim to unambiguously test the claim of dark matter detection by the DAMA experiments. DM-Ice17, consisting of 17 kg of NaI(Tl), has been continuously operating at a depth of 2457 m in the South Pole ice for over five years, demonstrating the feasibility of a low-background experiment in the Antarctic ice. Studies of low and high energy spectra, an annual modulation analysis, and a WIMP exclusion limit based on the physics run of DM-Ice17 are presented. We also discuss the plan and projected sensitivity of a new joint physics run, COSINE-100, with upgraded detectors at the Yangyang Underground Laboratory in Korea.

==> arxiv submission/acknowledgments.tex <==
\begin{acknowledgments}
The author would like to thank the conference organizers for the invitation at ICHEP2016. The DM-Ice collaboration thanks the Wisconsin IceCube Particle Astrophysics Center (WIPAC) and the IceCube collaboration for their on-going experimental support and data management. This work was supported in part by NSF Grants No.~PLR-1046816, PHY-1151795, and PHY-1457995, WIPAC, the Wisconsin Alumni Research Foundation, and Yale University. 

\end{acknowledgments}
